On the Analysis of Spatially Constrained Power of Two Choice Policies

We consider a class of power of two choice based assignment policies for allocating users to servers, where both users and servers are located on a two-dimensional Euclidean plane. In this framework, we investigate the inherent tradeoff between the communication cost, and load balancing performance of different allocation policies. To this end, we first design and evaluate a Spatial Power of two (sPOT) policy in which each user is allocated to the least loaded server among its two geographically nearest servers sequentially. When servers are placed on a two-dimensional square grid, sPOT maps to the classical Power of two (POT) policy on the Delaunay graph associated with the Voronoi tessellation of the set of servers. We show that the associated Delaunay graph is 4-regular and provide expressions for asymptotic maximum load using results from the literature. For uniform placement of servers, we map sPOT to a classical balls and bins allocation policy with bins corresponding to the Voronoi regions associated with the second order Voronoi diagram of the set of servers. We provide expressions for the lower bound on the asymptotic expected maximum load on the servers and prove that sPOT does not achieve POT load balancing benefits. However, experimental results suggest the efficacy of sPOT with respect to expected communication cost. Finally, we propose two non-uniform server sampling based POT policies that achieve the best of both the performance metrics. Experimental results validate the effctiveness of our proposed policies.

==> 00-abstract.tex <==
%%!TEX PS-program = pdflatexmk
%%!TEX root = spot.tex

We consider a class of power of two choice based assignment policies for allocating users to servers, where both users and servers are located on a two-dimensional Euclidean plane.  In this framework, we investigate the inherent tradeoff between the communication cost, and load balancing performance of different allocation policies. To this end, we first design and evaluate a \emph{Spatial Power of two} (sPOT) policy in which each user sequentially gets allocated to the least loaded server among its two geographically nearest servers. When servers are placed on a two-dimensional square grid, sPOT maps to the classical Power of two ({\it POT}) policy on the Delaunay graph associated with the Voronoi tessellation of the set of servers. We show that the associated Delaunay graph is $4$-regular and provide expressions for asymptotic maximum load using results from the literature. For uniform placement of servers, we map sPOT to a classical balls and bins allocation policy with bins corresponding to the Voronoi regions associated with the second order Voronoi diagram of the set of servers. We provide expressions for the lower bound on the asymptotic expected maximum load on the servers and prove that sPOT does not achieve POT load balancing benefits. However, experimental results suggest the efficacy of sPOT with respect to expected communication cost. Finally, we propose two non-uniform  server sampling based POT policies that achieve the best of both the performance metrics. Experimental results validate the effectiveness of our proposed policies.


%We solve the Euclidean matching problem, for one family of servers on a grid, and the second family chosen uniformly at random, when the cost depends on a power p of the Euclidean distance.

==> 04-perf.tex <==
In this section, we evaluate the performance of various allocation policies.
\subsection{Simulation Set up}
We consider $n = 2^6$ servers and equal number of users placed at a unit square uniformly at random. We ran $1000$ trials for each of the strategy and take the average maximum load, motivated by the procedure adopted in \cite{byers04}. For all the mobility models we take the maximum velocity to be $0.1$m/s and also consider the boundary effect by reflection. 
\subsection{Comparison of allocation policies}
\begin{figure}[htbp!]
\centering
\includegraphics[width=0.8\linewidth]{figs/plot_exp_load.png}
\caption{Comparison of various allocation policies.}
\label{fig:alloc}
\vspace{-0.1in}
\end{figure} 
We compare the performance of various allocation policies in Figure \ref{fig:alloc}. As expected, sPOO performs the worse while POT provides the least maximum expected load. Note that the introduction of spatial aspects into a policy increases the expected load. While sPOT is the second best policy, adding mobility to users does not effect the overall performance of sPOT. We study the effect of mobility in details, in the next Section. 

\subsection{Effect of mobility on sPOT}
In this section we discuss the effect of user and server mobility on performance of sPOT policy.
\subsubsection{Effect of user mobility}
We consider various mobility models \cite{camp02} to study its effect on maximum expected load behavior. We consider the effect of velocity on maximum expected load and present the results in Figure \ref{fig:vel_vs_load}. It is evident that even though the velocity was increased ten folds, the change in expected maximum load of the system was negligible. This suggests that mobility of users does not provide POT benefits.

\subsubsection{Effect of server mobility}
\begin{figure}[htbp!]
\centering
\includegraphics[width=0.8\linewidth]{figs/LoadVsVelocity.eps}
\vspace{-0.1in}
\caption{Effect of velocity on expected load.}
\label{fig:vel_vs_load}
\vspace{-0.1in}
\end{figure} 
We also consider mobile servers with static users. However, the expected load more or less remains the same as that of static server case.

==> 05a-rel-lit.tex <==
%%!TEX PS-program = pdflatexmk
%%!TEX root = spot.tex
\subsection{The classical balls and bins}
Holroyd et al. \cite{Holroyd09} first obtained upper and lower bounds on the expected request distance under stable matching policy for the case when users and servers are distributed according to a Poisson process on a $d$-dimensional spatial network. Abadi et al. \cite{Abadi17} were the first to derive bounds on expected request distance
for a unidirectional policy in a one-dimensional service network under Poisson distributed users and servers. They assume server capacity to be one in their analysis. Panigrahy et al. \cite{Panigrahy19} derived expressions for expected request distance in a more general setting where either users or servers are Poisson distributed and server capacities are greater than one. Our work complements and extends \cite{Panigrahy19} in the sense that we derive expressions for request distance distribution for a one-dimensional service network.

\subsection{Load Balancing on a Plane}

In the queueing theory field, there exists a vast volume of literature on the exceptional service queueing system. For example, \cite{Welch64, Pakes73, Baba99, Minh80} modeled the exceptional queueing system under different inter customer arrival time and service time distributions. However, theses works do not focus on batch service systems. For literature on non-accessible batch service queueing models with regular (non-exceptional) service, refer \cite{Downton55, bailey54}. \cite{Krishnamoorthy2000} discussed queue length distribution for an accessible regular batch service queueing system for different arrival and service time distributions. All of the above mentioned models either analyze exceptional service or accessible batch service queueing systems individually but not both. While authors in \cite{Panigrahy19} first derived the queue length distribution for an exceptional service accessible batch queueing system, we derive sojourn time distribution for such a system under Poisson customer arrival and general service time distribution.

\subsection{Distributed Service Network}

==> 05b-ack.tex <==
This research was sponsored by the U.S. ARL and the U.K. MoD under Agreement Number W911NF-16-3-0001 and by the NSF under Grant CNS-1617437. This document does not contain technology or technical data controlled under either the U.S. International Traffic in Arms Regulations or the U.S. Export Administration Regulations.% The views and conclusions contained in this document are those of the authors and should not be interpreted as representing the official policies, either expressed or implied, of the National Science Foundation, U.S. ARL or the U.K. MoD. 
